Indiscriminate Poisoning Attacks on Unsupervised Contrastive Learning

Indiscriminate data poisoning attacks are quite effective against supervised learning. However, not much is known about their impact on unsupervised contrastive learning (CL). This paper is the first to consider indiscriminate poisoning attacks of contrastive learning. We propose Contrastive Poisoning (CP), the first effective such attack on CL. We empirically show that Contrastive Poisoning, not only drastically reduces the performance of CL algorithms, but also attacks supervised learning models, making it the most generalizable indiscriminate poisoning attack. We also show that CL algorithms with a momentum encoder are more robust to indiscriminate poisoning, and propose a new countermeasure based on matrix completion. Code is available at: https://github.com/kaiwenzha/contrastive-poisoning.

==> src-new/fig-explain.tex <==
\begin{figure*}[h]
\begin{center}
\includegraphics[width=0.9\textwidth]{fig/explain-crop.pdf}
\vspace{-4mm}
\caption{
(a) Illustration of the poisoned encoder focusing a lot on the poisoning noise added to the image. (b) Histograms of the cosine distance between the embeddings of clean images and image with poisons (blue) or random noise (green). (c) Illustration of the poisoned encoder being tricked by the poisons to believe that two views of the same image is aligned. (d) Histograms of the cosine distance between the embeddings of two views of poisoned image (blue), clean images (orange), poisoning noise (gray).
}\label{fig:explain}
\end{center}
\end{figure*}

==> src-new/fig-loss-curve-wrap.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-10pt}
\includegraphics[width=0.59\textwidth]{fig/curve.pdf}
\vspace{-5pt}
\caption{Loss progression of training on poisoned dataset.} \vspace{-10pt}
\label{fig:loss-curve}
\end{wrapfigure}


==> src-new/fig-tsne-main.tex <==
\begin{figure}[t!]
\centering
\subfigure[EMP~(supervised)]{\includegraphics[width=0.3\columnwidth]{fig/tsne.ce.ues.pdf}}
\subfigure[EMP-CL~(SimCLR)]{\includegraphics[width=0.3\columnwidth]{fig/tsne.simclr.ues.pdf}}
\caption{t-SNE visualization of the sample-wise error-minimizing noise for supervised learning and SimCLR, on CIFAR-10. The noise is colored according to the class label of the corresponding sample. Accuracy of classifying the noise via linear logistic regression is displayed above the figure.}
\label{fig:tsne-main}
\end{figure}

==> src-new/tab-backup.tex <==

\begin{table}
\begin{minipage}{0.49\textwidth}
\caption{Attack performance as a function of the percentage of data that gets poisoned. 
 Experiment is conducted on CIFAR-10 with SimCLR.
 For reference, the table also shows the accuracy if the victim model is trained using only the $100\%-p$ clean samples.} \label{tab:poison-ratio}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
Percentage Poisoning ($p$) & 100\% & 90\% & 80\% & 50\%  & 20\%  & 10\% & 5\% \\ \midrule\midrule
\textsc{\small Clean Only~(100\%$-p$)}  & $-$ & 70.6 &	78.6 &	85.2 &	87.9 & & \\
\textsc{\small EMP-CL-C}   & 68.0 &  76.5 &	80.7 &	86.4 &	89.5 & 89.6 & 89.8 \\
\textsc{\small EMP-CL-S}       & 44.9 & 59.1 &	72.2 &	83.7	 & 88.1  & 88.6 & 89.6  \\
\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
\centering
\caption{Attack transferability across different neural network architectures. Attacker uses ResNet-18 to generate poisons. The victim uses SimCLR with various architectures: VGG-19, ResNet-18, ResNet-50, etc. Lower the accuracy, stronger the attack.}\label{tab:cross-arch}
\centering

\resizebox{\textwidth}{!}
{
\begin{tabular}{l ccccc}
\toprule
{Attack Type} & VGG-19 & ResNet-18 & ResNet-50 & DenseNet-121 & MobileNetV2 \\ 
\midrule\midrule
\textsc{None}   &  88.3     & 91.8 & 92.8 & 93.5 & 89.4    \\
\midrule
% \textsc{AP-CL}    &  78.0     & 80.2 & 84.4& 81.9 & 80.6\\
\textsc{EMP-CL-S}  &  35.1 & 44.9 & 49.1 & 48.4 & 42.6\\
\textsc{EMP-CL-C}  &  65.5 & 68.0 & 71.6 & 69.6 & 61.6 \\
\bottomrule
\end{tabular}
}
\end{minipage}

\end{table}

==> src-new/tab-cross-dataset.tex <==
\begin{table}[t]
\caption{Cross dataset (SimCLR).} \label{tab:cross-dataset}
\resizebox{0.49\textwidth}{!}
{
\begin{tabular}{l ccc}
\toprule
{Attacking dataset $\rightarrow$ Victim dataset} & Transfer & Oracle & Clean  \\ 
\midrule\midrule
\multicolumn{3}{l}{\emph{\textbf{CAP:}}} \\ \midrule
\textsc{CIFAR-10 $\rightarrow$ CIFAR-100}      & 58.3 & 46.9 &63.6     \\
\textsc{CIFAR-100 $\rightarrow$ CIFAR-10} & 89.6 & 80.2 &91.8 \\ \midrule\midrule
\multicolumn{3}{l}{\emph{\textbf{CUE-S:}}} \\ \midrule
\textsc{CIFAR-10 $\rightarrow$ CIFAR-100}      &  &  &     \\
\textsc{CIFAR-100 $\rightarrow$ CIFAR-10} & & & \\ \midrule\midrule
\multicolumn{3}{l}{\emph{\textbf{CUE-C:}}} \\ \midrule
\textsc{CIFAR-100 $\rightarrow$ ImageNet-100}      &  &  &     \\ 
\textsc{ImageNet-100 $\rightarrow$ CIFAR-100} & 58.9& & \\
\bottomrule
\end{tabular}
}
\end{table}

==> src-new/understand.tex <==
\input{src-new/fig-explain}

In this paragraph, we answer the question: how our contrastive poisoning attacks the CL algorithm and tricks it to learn bad features. As designed, the contrastive poisons is supposed to help the CL algorithm to cheat the learning criterion of contrastive learning during training. Considering contrastive learning objective (e.g. InfoNCE), as pointed out in \citep{wang2020understanding}, can be interpreted as a combination of \emph{alignment} (aligning different views of the same image) and \emph{uniformity} (spreading features to maximize the information), one could ask which part of the CL objectives gets shortcuted. Is it alignment or uniformity or both? Intuitively, shortcutting uniformity is hard since it means the poisons make the encoder uniformly distribute the poisoned images (in the embeddings space) while distributing the clean image in a highly ununiform way (e.g. collapsing them to a point). In contrast, shortcutting alignment is more straightforward, i.e., the poisoning noise becomes a hint of the encoder to align the two augmented views of the same poisoned image. If the encoder rely on the hint too much, it will fail miserably on aligning clean images since there is not such hint in the clean data. We confirm our intuition by the following analysis.
We monitor the progression of the loss values of a model trained on poisoned dataset. We monitor three losses, InfoNCE, alignment and uniformity. We compare each loss computed on the poisoned images versus that computed on the clean images. As the result shown in \Figref{fig:loss-curve}, the alignment get shortcuted significatnly as there exists a huge gap between the poisoned alignment values (blue curve) and clean alignment values (orange curve). In contrast the gap is much less for the uniformity. The curves in \Figref{fig:loss-curve} is for class-wise CP attacking SimCLR. The results for sample-wise CP is similar (see \Appref{}).

Now we go deeper an ask how exactly CP shortcut the alignment loss? Does it really work as a hint as we thought? The answer is yes. Supported by our analysis, we argue two points: first, CP causes the encoder to focus a lot on the poisoning noise while paying less attention on the true image; second, CP noise itself has a strong invariance to the data augmentation, which helps the encoder put two views of the image with the same poisoning noise next to each other in the embedding space. 

\Figref{fig:explain}(a) illustrates how we test the first point. Consider a clean image $x$, its poisoning noise $\delta$, a random bounded noise $r$ and encoder $f$. We show in the embedding space, the poisoned image $f(x+\delta)$ has a significantly longer distance to the clean image $f(x)$ compared with a randomly perturbed image $f(x+r)$. \Figref{fig:explain}(b) shows the histograms of the cosine distance between the embeddings.  We can see that the poisoned image most of the time having a $1$ cosine distance from the clean image meaning they are orthogonal. In contrast, a random noise only perturb the embedding in the neighbourhood of the clean image leading to a cosine distance close to $0$.

\Figref{fig:explain}(c) illustrates how we test the second point. Let $a_1, a_2$ be the two augmentation and $d$ be the cosine distance. We now compare the cosine distance (in the embedding space) between two views of a poisoned image $d_1=d(f(a_1(x)),f(a_2(x)))$, a clean image $d_2=d(f(a_1(x+\delta)),f(a_2(x+\delta)))$, the poisoning noise $d_2=d(f(a_1(\delta)),f(a_2(\delta)))$. We show the histograms of $d_1$ (blue), $d_2$ (orange), $d_3$ (gray) in \Figref{fig:explain}(d). It is not surprised that $d_1$ be small and $d_2$ be large because we expect it according to the alignment loss curve shown before. What interesting is that $d_3$ is also relatively small. From the figure, we can see most of the time it is lower than $0.2$. It means even if the encoder only see the two augmentation of the same poisoning noise, it tend to map it to the same embedding, i.e., from the perspective of the encoder, the poisoning noise is invariant under the augmentation. 
